Bounding elastic photon-photon scattering at $\sqrt s \approx 1\,$MeV using a laser-plasma platform

We report on a direct search for elastic photon-photon scattering using x-ray and $\gamma$ photons from a laser-plasma based experiment. A gamma photon beam produced by a laser wakefield accelerator provided a broadband gamma spectrum extending to above $E_\gamma = 200$ MeV. These were collided with a dense x-ray field produced by the emission from a laser heated germanium foil at $E_x \approx 1.4$ keV, corresponding to an invariant mass of $\sqrt{s} = 1.22 \pm 0.22$ MeV. In these asymmetric collisions elastic scattering removes one x-ray and one high-energy $\gamma$ photon and outputs two lower energy $\gamma$ photons. No changes in the $\gamma$ photon spectrum were observed as a result of the collisions allowing us to place a 95% upper bound on the cross section of $1.5 \times 10^{15}\,\mu$b. Although far from the QED prediction, this represents the lowest upper limit obtained so far for $\sqrt{s} \lesssim 1$ MeV.

==> authors-PLB.tex <==
% commands for each institution  
\newcommand{\IC}{The John Adams Institute for Accelerator Science, Imperial College London, London, SW7 2AZ, UK}

\newcommand{\UMICH}{Center for Ultrafast Optical Science, University of Michigan, Ann Arbor, MI 48109-2099, USA}

\newcommand{\DESY}{Deutsches Elektronen-Synchrotron DESY, Notkestr. 85, 22607 Hamburg, Germany}

\newcommand{\QUB}
{School of Mathematics and Physics, Queen's University of Belfast, BT7 1NN, Belfast, UK}

\newcommand{\HIJENA}
{Helmholtz Institut Jena, Fr\"{o}belstieg 3, 07743 Jena, Germany}

\newcommand{\JENA}
{Institut f\"{u}r Optik und Quantenelektronik, Friedrich-Schiller-Universit\"{a}t, 07743 Jena, Germany}

\newcommand{\CLF}{Central Laser Facility, STFC Rutherford Appleton Laboratory, Didcot OX11 0QX, UK}

\newcommand{\YORK}{Department of Physics, University of York, York, YO10 5DD, UK}

\newcommand{\OXFORD}{Department of Physics, University of Oxford, Oxford, OX1 3PU, UK}

\newcommand{\AWE}{AWE Aldermaston, Reading RG7 4PR, UK}

\newcommand{\CELIA}{Université de Bordeaux-CNRS-CEA, Centre Lasers Intenses et Applications (CELIA), UMR 5107, F-33405 Talence, France}

\newcommand{\UVa}{Departamento de Física Teórica Atómica y Óptica, Universidad de Valladolid, 47011 Valladolid, Spain}

\newcommand{\LBNL}{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, US}

\newcommand{\LANC}{Physics Department, Lancaster University, Lancaster LA1 4YB, UK}

\newcommand{\CERN}{CERN, Geneva, Switzerland}
\newcommand{\PLYMOUTH}{Centre for Mathematical Sciences, University of Plymouth, PL4 8AA, UK}






\author[imp]{R.~Watt}
\author[imp]{B.~Kettle}
\author[imp]{E.~Gerstmayr}
\author[ply]{B.~King}
\author[qub]{A.~Alejo}
\author[clf]{S.~Astbury}
\author[york]{C.~Baird}
\author[desy]{S.~Bohlen}
\author[cern]{M.~Campbell}
\author[imp]{C.~Colgan}
\author[cern]{D.~Dannheim}
\author[clf]{C.~Gregory}
\author[hijena,jena]{H.~Harsh}
\author[oxf]{P.~Hatfield} 
\author[umich]{J.~Hinojosa}
\author[hijena,jena]{D.~Hollatz}
\author[clf]{Y.~Katzir}
\author[awe]{J.~Morton}
\author[york]{C.D.~Murphy}
\author[cern]{A.~Nurnberg}
\author[desy]{J.~Osterhoff}
\author[uva]{G.~P\'erez-Callejo}
\author[desy]{K.~P\~{o}der}
\author[clf]{P.P.~Rajeev}
\author[hijena]{C.~Roedel}
\author[jena]{F.~Roeder}
\author[hijena,jena]{F.C.~Salgado}
\author[qub]{G.M.~Samarin}
\author[qub]{G.~Sarri}
\author[hijena,jena]{A.~Seidel}
%S.~Spannagel\cern$^,$\desy,  %asked to be removed
\author[clf]{C.~Spindloe}
\author[lbnl]{S.~Steinke}
\author[qub,lanc]{M.J.V.~Streeter}
\author[umich,lanc]{A.G.R.~Thomas}
\author[york]{C.~Underwood}
\author[imp]{W.~Wu}
\author[hijena,jena]{M.~Zepf}
\author[imp]{S.J.~Rose}
\author[imp]{S.P.D.~Mangles}


\affiliation[imp]{organization=\IC}
\affiliation[ply]{organization=\PLYMOUTH}

\affiliation[umich]{organization=\UMICH}
\affiliation[desy]{organization=\DESY}
\affiliation[qub]{organization=\QUB}
\affiliation[hijena]{organization=\HIJENA}

\affiliation[jena]{organization=\JENA}
\affiliation[clf]{organization=\CLF}
\affiliation[york]{organization=\YORK}
\affiliation[oxford]{organization=\OXFORD}

\affiliation[awe]{organization=\AWE}
\affiliation[celia]{organization=\CELIA}
\affiliation[uva]{organization=\UVa}
\affiliation[lbnl]{organization=\LBNL}


\affiliation[lanc]{organization=\LANC}
\affiliation[cern]{organization=\CERN}










\vspace{10pt}

